Stop talking to me -- a communication-avoiding ADER-DG realisation

We present a communication- and data-sensitive formulation of ADER-DG for hyperbolic differential equation systems. Sensitive here has multiple flavours: First, the formulation reduces the persistent memory footprint. This reduces pressure on the memory subsystem. Second, the formulation realises the underlying predictor-corrector scheme with single-touch semantics, i.e., each degree of freedom is read on average only once per time step from the main memory. This reduces communication through the memory controllers. Third, the formulation breaks up the tight coupling of the explicit time stepping's algorithmic steps to mesh traversals. This averages out data access peaks. Different operations and algorithmic steps are ran on different grid entities. Finally, the formulation hides distributed memory data transfer behind the computation aligned with the mesh traversal. This reduces pressure on the machine interconnects. All techniques applied by our formulation are elaborated by means of a rigorous task formalism. They break up ADER-DG's tight causal coupling of compute steps and can be generalised to other predictor-corrector schemes.

==> a8a_raw-data.tex <==
\section{Experiments' raw data}

\subsection{Shared memory}

\begin{figure}
 \begin{center}
   \includegraphics[scale=0.8]{experiments/simulation/hamilton/Euler_ADERDG/multicore-results-3d/generic/Euler_ADERDG-no-output-updates-regular-0-linear.pdf}
   \includegraphics[scale=0.8]{experiments/simulation/hamilton/Euler_ADERDG/multicore-results-3d/generic/Euler_ADERDG-no-output-updates-regular-1-linear.pdf}
 \end{center}
 \caption{
  Shared memory, $d=3$ on Broadwell for $27\times27\times27$
  (left) and $81\times81\times81$ (right).
  \label{results:appendix:multicore:broadwell}
 }
\end{figure}

The Broadwell results (Fig.~\ref{results:appendix:multicore:broadwell}) show
ragged stand strong speedup behaviour.
We note that $p=9$ does not fit on our Broadwell nodes for a
$81\times81\times81$ as it exceeds the main memory.
The speedup curves close once the mesh becomes finer. 

\begin{figure}
 \begin{center}
   \includegraphics[scale=0.8]{experiments/simulation/archer/Euler_ADERDG/multicore-results-3d/Euler_ADERDG-no-output-updates-regular-0-linear.pdf}
   \includegraphics[scale=0.8]{experiments/simulation/archer/Euler_ADERDG/multicore-results-3d/Euler_ADERDG-no-output-updates-regular-1-linear.pdf}
 \end{center}
 \caption{
  Shared memory, $d=3$ on KNL for $27\times27\times27$
  (left) and $81\times81\times81$ (right).
  \label{results:appendix:multicore:knl}
 }
\end{figure}

The KNL behaviour (Fig.~\ref{results:appendix:multicore:knl}) is qualitatively
similar to the Broadwell data but way smoother.
Here, we do see strong speedup, i.e.~the bigger problem scales better.


